Semantic Operators: A Declarative Model for Rich, AI-based Data Processing

The semantic capabilities of large language models (LLMs) have the potential to enable rich analytics and reasoning over vast knowledge corpora. Unfortunately, existing systems either empirically optimize expensive LLM-powered operations with no performance guarantees, or serve a limited set of row-wise LLM operations, providing limited robustness, expressiveness and usability. We introduce semantic operators, the first formalism for declarative and general-purpose AI-based transformations based on natural language specifications (e.g., filtering, sorting, joining or aggregating records using natural language criteria). Each operator opens a rich space for execution plans, similar to relational operators. Our model specifies the expected behavior of each operator with a high-quality gold algorithm, and we develop an optimization framework that reduces cost, while providing accuracy guarantees with respect to a gold algorithm. Using this approach, we propose several novel optimizations to accelerate semantic filtering, joining, group-by and top-k operations by up to $1,000\times$. We implement semantic operators in the LOTUS system and demonstrate LOTUS' effectiveness on real, bulk-semantic processing applications, including fact-checking, biomedical multi-label classification, search, and topic analysis. We show that the semantic operator model is expressive, capturing state-of-the-art AI pipelines in a few operator calls, and making it easy to express new pipelines that match or exceed quality of recent LLM-based analytic systems by up to $170\%$, while offering accuracy guarantees. Overall, LOTUS programs match or exceed the accuracy of state-of-the-art AI pipelines for each task while running up to $3.6\times$ faster than the highest-quality baselines. LOTUS is publicly available at https://github.com/lotus-data/lotus.

==> algs/formatting.tex <==
\DontPrintSemicolon
% \small

\SetKwIF{If}{ElseIf}{Else}{if}{}{else if}{else}{endif}
\SetKwFor{For}{for}{}{}
\SetKwFor{ForEach}{for each}{}{}
\LinesNumbered


==> tables/filter-ablation.tex <==
\begin{table*}[h]

\centering
\caption{Fact-checking Semantic Filter Cascades Evaluation. \sid{To be plotted. Data here is old - correct data in the google colab}}
\vspace{-.3cm}
\begin{tabular}{cccc}
% \hline
\toprule
Method & Accuracy & QPS \\
% \hline
\midrule
Llama-70B & 90.6 & 3.17 \\
Llama-8B & 87 & XX \\
Tiny-Llama & 73.2 & 9.70 \\
Llama 8B, 70B (conf\_tresh=0.9)  & 90.0 & 7.85 \\
Llama 8B, 70B (conf\_tresh=0.99)  & 90.6 & 5.56\\
Llama 8B, 70B (conf\_tresh=0.9)  & 90.8 & 4.08 \\
Tiny-llama, Llama 70B (conf\_tresh=0.5)  & 74.8 & 9.03 \\
Tiny-llama, Llama 70B (conf\_tresh=0.6)  & 84.8 & 5.33\\
Tiny-llama, Llama 70B (conf\_tresh=0.7)  & 89.4 & 3.49 \\
Tiny-llama, Llama 70B (conf\_tresh=0.8)  & 90.6 & 3.00 \\

% \hline
\bottomrule
\label{tab:filtercascades}

\end{tabular}
% \vspace{-.4cm}

\end{table*}


==> tables/operators_short.tex <==
\begin{small}
\begin{table*}[!t]
\newcolumntype{C}[1]{>{\raggedright\arraybackslash}p{#1}}
\renewcommand{\arraystretch}{1.4} % Adjust the value to increase/decrease row spacing
\centering
\caption{Summary of Key Semantic Operators. $T$ denotes a relation, $X$ and $Y$ denote arbitrary tuple types, $L[X]$ denotes a list of elements with type $X$, and $A$ denotes the type of a particular column or attribute. $l$ denotes a parameterized natural language expression (``langex" for short), which takes tuples as input and performs a function such as a predicate, an aggregation, a comparator, or a projection, depending on the operator's signature. \rev{Each operator may permit optional parameters to set accuracy targets, as described in Section~\ref{sec:impl}.}}
\vspace{-.3cm}
\begin{tabular}{C{6cm}C{11cm}}
% \hline
\toprule
\textbf{Operator} & \textbf{Description} \\
% \hline
\midrule
$\mathit{sem\_filter}(l\textit{: } X \rightarrow \mathit{Bool})$ & Returns the tuples in a table that pass the provided langex predicate. \\
% \hline
$\mathit{sem\_join}(t\textit{: } T \comma l\textit{: } (X, Y) \rightarrow \mathit{Bool})$ & Joins a table against a second table $t$ by keeping all pairs of tuples that pass the provided langex predicate. \\
% \hline
$\mathit{sem\_agg}(l\textit{: } L[X] \rightarrow \mathit{X})$ & Performs an aggregation over the input tuples according to the langex, which specifies a commutative, associative aggregation function over a list of tuples. \\
% \hline
$\mathit{sem\_topk}(l\textit{: } L[X] \rightarrow L[X]\comma k\textit{: }int)$ & Ranks each tuple and returns the $k$ best according to the langex, which specifies a ranking function that sorts a list of tuples. \\
% \hline
$\mathit{sem\_group\_by}(l\textit{: } X \rightarrow Y\comma C\textit{: } int)$ & Groups the tuples into $C$ categories based on the langex, which specifies a grouping criteria. \\
$\mathit{sem\_map}(l\textit{: } X \rightarrow Y)$ & Performs a projection, returning a new column, according to the provided langex. \\
% $\mathit{sem\_search}(l:X \rightarrow q\comma k\textit{: } int\comma a: A)$ & Performs a top-$k$ search over column $a$ using the langex, which is a constant function providing the query expression $q$.
\\

% \hline
\bottomrule
\label{tab:operators}

\end{tabular}
\vspace{-1.0cm}

\end{table*}

% \hline
% $\mathit{sem\_cluster\_by}(a\textit{: } A\comma C\textit{: } \mathit{int})$\liana{remove?} & Performs a semantic similarity-based clustering  over column $a$ to create $C$ groups. \\
% $\mathit{sem\_index}(a\textit{: } A \comma{} \mathit{path} \textit{: } \mathit{String})$ & Creates similarity index for column $a$ and saves to path. \\
% $load\_sem\_index(k: K, path: String)$ & loads similarity index for column $k$ form path \\
% $\mathit{sem\_partition\_by}(f\textit{: } X \rightarrow int)$ & Applies the partitioner function, $f$ over the table to specify a grouping that overrides associativity assumptions for operations like \verb|sem_agg|. \\
% \hline
% $\mathit{sem\_extract}(l\textit{: } X \rightarrow Y)$ & Performs a projection according to the langex, returning a column with a list of substrings from the input tuples. \liana{this can also move to api}\\
% \hline



\end{small}


==> tables/papers.tex <==
\begin{figure*}[!t]
  \centering
  % \vspace{-.4cm}
  \includegraphics[width=0.8\linewidth]{figures/papers_schema.png}
  \vspace{-.4cm}
  \caption{\small Table schema of ArXiv papers.}
  \label{fig:papers}
   % \vspace{-.3cm}
\end{figure*}



==> tables/sem_group_by.tex <==
\begin{footnotesize}
    

\begin{table}[t]

\centering
\caption{Discovered Group Labels Over ArXiv Papers}
\vspace{-.3cm}
\begin{tabular}{c}
% \begin{tabular}{p{6cm}p{1.1cm}p{.8cm}}
% \hline
\toprule
% Label\\
% % \hline
% \midrule
($\mu_1$) Advancements in Recommender Systems and Multimodal Data Integration\\

($\mu_2$) Advancements in Generative Information Retrieval Systems\\

($\mu_3$) Advancements in Large Language Models for Various Applications\\

($\mu_4$) Advancements in AI Security and Malware Detection Techniques\\

($\mu_5$) Advancements in Robotic Navigation and Manipulation Techniques\\
\bottomrule
\label{tab:groupby}

\end{tabular}
\vspace{-.5cm}

\end{table}

\end{footnotesize}
    


==> tables/topk-cifar.tex <==
% \usepackage{booktabs}
% \usepackage{multirow}

% \begin{small}
    
% \begin{table}[t]
% \centering
% \caption{Ranking Results on CIFAR- \& HellaSwag-bench}
% \vspace{-.2cm}
% % \begin{tabular}{ccccc}
% \begin{tabular}{p{3cm}p{1.2cm}p{.8cm}p{1.2cm}p{.8cm}}
% \toprule    
% \multirow{2}{*}{Method} & \multicolumn{2}{c}{CIFAR} & \multicolumn{2}{c}{HellaSwag} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5}
% & nDCG@10  & ET (s) & nDCG@10  & ET (s)\\
% \midrule
% Search & 0.252 & 0.008 & 0.119 & 0.008 \\
% Search + Reranker & 0.001 & 2.57 & 0.461 & 2.36 \\
% \sys Top-k - Llama 70B & 0.710 & 39.6  & 0.975 & 63.6 \\
% DocETL - Llama 70B & TODO & TODO & .252 & TODO \\
% DocETL - GPT 4o mini & TODO & TODO & .183 & TODO \\
% UDF ie pointwise ranking & TODO & TODO & TODO & TODO \\
% \bottomrule
% \end{tabular}
% \label{tab:ranking_cifar}
% \end{table}
% % \vspace{-.5cm}


% \end{small}



\begin{small}
    
\begin{table}[t]
\centering
\caption{Old Ranking Results on CIFAR- \& HellaSwag-bench}
\vspace{-.2cm}
% \begin{tabular}{ccccc}
\begin{tabular}{p{3cm}p{1.2cm}p{.8cm}p{1.2cm}p{.8cm}}
\toprule    
\multirow{2}{*}{Method} & \multicolumn{2}{c}{CIFAR} & \multicolumn{2}{c}{HellaSwag} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5}
& nDCG@10  & ET (s) & nDCG@10  & ET (s)\\
\midrule
Search & 0.252 & 0.008 & 0.119 & 0.008 \\
Search + Reranker & 0.001 & 2.57 & 0.461 & 2.36 \\
LLM UDF & TODO & TODO & 0.0912 & 19.7 \\
\sys Top-k - Llama 70B & TODO & TODO  & 0.919 & 57.0 \\
DocETL - Llama 70B & TODO & TODO & .252 & TODO \\
DocETL - GPT 4o mini & TODO & TODO & .183 & TODO \\

\bottomrule
\end{tabular}
\label{tab:ranking_cifar}
\end{table}
% \vspace{-.5cm}


\end{small}







==> tables/topk-scifact.tex <==
\begin{small}
    
\begin{table}[t]

\centering
\caption{Ranking Results on SciFact \liana{add UDF with pointwise ranking}}
\vspace{-.3cm}
% \begin{tabular}{ccc}
\begin{tabular}{p{4cm}p{1.1cm}p{.8cm}}
% \hline
\toprule
Method & nDCG@10  & ET (s)\\
% \hline
\midrule
Search & 0.712 & 0.009 \\
Search + Reranker & 0.741 & 2.64 \\
LLM UDF & 0.458 & 9.83 \\
DocETL - Llama-70B + 4o optimizer  & 0.531 & TODO \\
\sys - Llama-70B & 0.768 & 36.2 \\
% \sys - GPT-4o & 0.800 & 11.2 \\
\bottomrule
\label{tab:ranking_scifact}

\end{tabular}
\vspace{-.6cm}

\end{table}

\end{small}

